PALT: Parameter-Lite Transfer of Language Models for Knowledge Graph Completion

This paper presents a parameter-lite transfer learning approach of pretrained language models (LM) for knowledge graph (KG) completion. Instead of finetuning, which modifies all LM parameters, we only tune a few new parameters while keeping the original LM parameters fixed. We establish this via reformulating KG completion as a "fill-in-the-blank" task, and introducing a parameter-lite encoder on top of the original LMs. We show that, by tuning far fewer parameters than finetuning, LMs transfer non-trivially to most tasks and reach competitiveness with prior state-of-the-art approaches. For instance, we outperform the fully finetuning approaches on a KG completion benchmark by tuning only 1% of the parameters. The code and datasets are available at \url{https://github.com/yuanyehome/PALT}.

==> chap/misc.tex <==

% The triplet with a missing entity is cast into a cloze statement and fed into the pretrained LM to trigger related knowledge. With all the original parameters fixed, this formulation achieves non-trivial zero-shot results. 
% To further adapt LMs to KG completion, we design several essential and novel architectures
% , one in the middle and one in the last layer
% We find that the linear projection is effective and efficient in calibrating knowledge. 



% Our models under the same model architect obtains state-of-the-art or competitive KG completion performance compared to the fully finetuning approaches on all KG completion tasks with the same model architecture.  %We enable zero-shot transfer of the knowledge that the pretrained LMs have about the KG completion tasks by keeping the original parameters frozen.
% There are some works focus on few-shot transfer of pretrained LMs~\cite{he2021empirical}, but to the best of our knowledge, our work is the first to enable zero-shot transfer of pretrained LMs to KG completion.
% \vspace{-0.1in}
% \item We enable zero-shot transfer of the knowledge that LMs know about the KG completion via answering questions in fill-in-the-blank cloze statements. 

% \todo{separate finetuning, task-specifc standard model, finetuning general model, and their corresponding results}
% without changing any LM parameters

% They use Transformer~\cite{Vaswani_attention} as the base model architecture and are pretrained on a large corpus. Because of the powerful representation ability of Transformer and abundant information from the training corpus, pretrained LMs are able to learn general knowledge. 

% However, applying these methods to KG completion is non-trivial. 
% P-Adapters~\cite{newman_p-adapters:_2021} insert an adapter between the embedding layer and the first attention layer to query knowledge. However, it relies on a single \textspt{[MASK]} output and does not generalize to other tasks like KG completion. 

% In general, we focus on transferring pretrained LMs to KG completion, which is not straightforward since the KG is not represented by natural language. 

% knowledge-intensive 

% For example, TransE~\cite{TransE} uses a translation distance. Some other approaches use tensor factorization~\cite{Rescal, Tucker}, convolution~\cite{ConvE, ConvKB} and adversarial training~\cite{cai_kbgan:_2018}. 

% Previous work has shown it is possible to leverage pretrained LMs for knowledge probing~\cite{he2021empirical, LAMA}. They design a template for each task and query knowledge by filling a special mask token. This approach only fits for querying knowledge with one token. In more general cases, the number of tokens is unknown, so mask based prediction is not applicable. Our proposed \method\ has no such limitation. It takes advantage of next sentence prediction and works for knowledge with any number of tokens. TEKE~\cite{wang_text-enhanced_2016} incorporates rich textual context information to expand the semantic structure of the KG. 


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.4\textwidth]{fig/error_case.png}
%     \vspace{-0.05in}
%     \caption{An error case of \method . The tail entity ``barbiturate'' is a rare word so the attention weights on it are small, leading to an error.\yuanye{add visualization on a high-error ratio relation and a low-error ratio relation}}
%     \label{fig:error}
% \end{figure}


% \section{Introduction}
% Knowledge graphs are structured representations of factual knowledge to help machines better understand and reasoning in the real world scenario~\cite{bollacker_freebase:_2008}. They typically consist of triplets in the form of (head entity, relation, tail entity), indicating that the relation holds between the head and tail entities. There are lots of applications using knowledge graphs and achieving great success, such as question answering~\cite{Guu2015TraversingKG,hao_end--end_2017} and web search~\cite{Xiong2017ExplicitSR}.

% An important factor that affects knowledge graphs is incompleteness~\cite{Carlson2010TowardAA,Dong2014KnowledgeVA}. Large-scale knowledge graphs usually rely on automatic machine construction and thus inevitably suffer from missing entities and relations. Therefore, knowledge graph completion, the task of predicting a missing entity or relation given an incomplete triplet, plays a crucial role and attracts much attention in this domain~\cite{TransE, RotateE, KGBERT}. Traditional approaches mainly treat each entity as a node and relation as a link and encode the structure information by graph representation learning~\cite{TransE, TransH, TransR}. However, natural language description of entities and relations also contains rich information and should be useful for knowledge completion. KG-BERT~\cite{KGBERT} leverages BERT~\cite{BERT}, a pre-trained language model, to encode text description for knowledge completion and achieves a great success. However,  this approach fine-tunes the whole language model, which requires a large amount of computational and storage resource.

% In this work, we propose \method, a method that transfers {\bf P}re-trained {\bf L}anguage models for {\bf E}fficient knowledge {\bf C}ompletion. Specifically, we argue that the knowledge completion task fits well with the next sentence prediction task of pre-training. Thus, we prepare the triplet description as a sentence pair just like pre-training and directly make use of the NSP classifier to score the triplet. To efficiently transfer knowledge in the pre-trained language model for the completion task, we first add a knowledge prompt encoder at the input layer to recall related knowledge. Then we add knowledge calibration encoders in the middle and end of the language model, which prepare the internal knowledge needed for the knowledge graph completion task. We keep all the language model parameters fixed and only tune these light-weighted knowledge prompt and calibration encoders. We show that with less optimization and storage burden than fine-tuning, our method can still achieve competitive performance.

% The contributions of our work are two-fold:
% \begin{itemize}
%     \vspace{-0.1in}
%     \item We design \method, an efficient knowledge graph completion method which leverages a pre-trained language model to encode text description of entities and relations. We are the first to formalize the knowledge graph completion task as the next sentence prediction and use NSP classifier to score the triplet. Different from fine-tuning, we add a \prompt\ and \calibration\ s to efficiently recall and calibrate the knowledge in the pre-trained language model for knowledge graph completion task.
%     \vspace{-0.1in}
%     \item We test \method\ on 5 datasets of 2 knowledge completion tasks. With only 1.6\% tunable parameters of fine-tuning, \method\ can still achieve competitive or better performance.
% \end{itemize}









The zero-shot approach is on the left, where the knowledge graph completion task is framed as textual entailment and fed into BERT as a sentence pair. The input is aligned with that of NSP during pre-training and the output of the NSP classifier on \textspt{[CLS]} token is treated as the confidence score of the triplet. To improve the transfer ability, we add two kinds of adapting layers on the right. We first insert prompt tokens into the input and a \prompt\ on top of the token embedding to recall related knowledge. Then two \calibration s are added in the middle and end of Transformer layers to prepare the knowledge for the knowledge graph completion task. Only parameters in dashed frames are tunable and those in solid frames are fixed.


% Fine-tuning is the prevalent way to transfer pre-trained language models for downstream tasks, which has been a great success recently. However, it updates all language model parameters and thus requires a large amount of computational and storage resources. Some alternative ways are proposed but they have not been applied to tasks in structured domain like knowledge graph completion yet. In this work, we propose \method , an efficient way to transfer pre-trained language models for the knowledge graph completion task. We first formalize the knowledge completion task as next sentence prediction task (NSP) and directly make use of the NSP classifier for triplet scoring. We fix the pre-trained language model and only add a small fraction of tunable parameters to recall and calibrate related knowledge. With less optimization and storage burden than fine-tuning, our method can still achieve competitive performance.\yuanye{add code}


% Completing knowledge triples is a fundamental problem for knowledge graph. Natural language description of entities and relations contains rich information but how to leverage it for knowledge graph completion efficiently is not well explored yet. KG-BERT treats the knowledge graph completion task as a text binary classification task, and solves it by fine-tuning a pre-trained BERT. However, this approach updates all language model parameters and thus requires large computation and storage resources. In this work, we propose \method, an efficient way for knowledge graph completion with pre-trained language models. We first formalize the knowledge completion task as next sentence prediction task (NSP) and directly make use of the NSP classifier for triplet scoring. To efficiently transfer related knowledge for the completion task, we add a \prompt\ and \calibration s on pre-trained language models while keep all language model parameters fixed. The \prompt\ assumes that a continuous prompt enhanced input can more effectively recall the knowledge in the language models, while the \calibration\ prepares the internal knowledge needed for the knowledge graph completion task. With less optimization and storage burden than fine-tuning, our method can still achieve competitive performance.

% \jianhao{revise according to the abstract}
% Transferring pre-trained language models (PLMs) for downstream tasks has shown great success in natural language processing. Benefiting from the large corpus and powerful model architecture, PLMs learn not only syntactic~\cite{hewitt-manning-2019-structural} and semantic representations~\cite{brown_language_2020}, but also commonsense~\cite{davison-etal-2019-commonsense} and world knowledge~\cite{petroni-etal-2019-language}.

% The prevalent way to use PLMs is fine-tuning, where all language model parameters are updated and stored for each downstream task. This paradigm is expensive due to the requirement of a great amount of computational and storage resources, especially for large models. Recently, some alternative ways are proposed to efficiently transfer PLMs for downstream tasks, including prompt-tuning~\cite{shin-etal-2020-autoprompt, liu_gpt_2021} and adaptors~\cite{pmlr-v97-houlsby19a, k-adapter}. However, these methods mainly focus on traditional NLP tasks like text classification, question answering and summarization, but have not been applied to structured domains like knowledge graph completion yet. A recent work shows that PLMs are useful for knowledge graph completion and achieves great performance~\cite{KGBERT}, but it still follows the fine-tuning approach and is thus not efficient.

% \jianhao{highlight the novelty of the approach}
% In this work, we propose \method, a {\bf P}arameter-{\bf E}fficient {\bf T}ransfer learning of pre-trained language models for knowledge graph completion. Different from fine-tuning, \method\ keeps all language model parameters fixed. To narrow the gap between pre-trained language models and knowledge graph completion, we frame knowledge graph completion as a standard natural language understanding task. We align input and output with those during pre-training, and thus enable zero-shot transfer of the language models to knowledge graph completion tasks. This zero-shot approach already gives a good performance. To better adapt PLMs to these tasks, we add light-weighted layers to recall and calibrate related knowledge. We show that by tuning a few parameters independently, language models transfer non-trivially to most tasks and can reach competitiveness with prior state-of-the-art approaches. 


% In this work, we propose \method, a method that transfers PLMs with {\bf P}rompting and c{\bf A}librating for knowledge graph {\bf C}ompl{\bf E}tion. Different from fine-tuning, \method\ keeps all language model parameters fixed and only adds a small fraction of tunable parameters. Specifically, we notice that the knowledge completion task fits well with the next sentence prediction (NSP) task of pre-training. Thus, we first prepare the triplet description as a sentence pair just like pre-training and directly make use of the NSP classifier to score the triplet. Furthermore, to efficiently transfer knowledge in the pre-trained language model, we append virtual prompts into the input sequences and transform the token embeddings. These prompts can recall related knowledge from the input embeddings and the transformation helps the following attention layers to better leverage such knowledge. After that, we add another two linear mappings in the middle and the last layer to calibrate the knowledge for the completion task. We show that with far less tunable parameters than fine-tuning, our method can still achieve competitive performance.


% We argue that the knowledge completion task fits well with the next sentence prediction (NSP) task of pre-training. Thus, we prepare the triplet description as a sentence pair just like pre-training and directly make use of the NSP classifier to score the triplet. To efficiently transfer knowledge in the pre-trained language model for the completion task, we first add a knowledge prompt encoder at the input layer to recall related knowledge. Then we add knowledge calibration encoders in the middle and end of the language model, which prepare the internal knowledge needed for the knowledge graph completion task. We keep all the language model parameters fixed and only tune these light-weighted knowledge prompt and calibration encoders. We show that with less optimization and storage burden than fine-tuning, our method can still achieve competitive performance.

% The contributions of our work are two folds:
% \begin{itemize}
%     \vspace{-0.1in}
%     \item We design \method, a parameter-efficient transfer learning for knowledge graph completion which leverages a fixed pre-trained language model. We formalize knowledge graph completion task as a standard natural language understanding task and enable zero-shot transfer. We further add light-weighted layers and tune these layers independently with all language model parameters fixed. 
%     \vspace{-0.1in}
%     \item We test \method\ on 5 datasets of 2 knowledge completion tasks. With only 1.6\% tunable parameters of fine-tuning, \method\ can still achieve competitive or better performance.
% \end{itemize}

% \jianhao{adjust the structure of the approach: first introduce zero-shot PET; then introduce PET with prompt and calibration; add motivating examples to illustrate the approach, and highlight the difference/novelty of the approach}

% \jianhao{textual entailment; task of interest; in-distribution and out-of-distribution knowledge->domain adaption (prompt: input to modle knowledge adaption; calibration: model knowledge to task adaptation.)}
% We propose \method, a {\bf P}arameter-{\bf E}fficient {\bf T}ransfer of pre-trained language models for knowledge graph completion. Different from fine-tuning which requires updating all language model parameters, \method\ keeps the PLM fixed and only tunes a few or even no parameters. The success of such efficient transfer mainly relies on our formulation where knowledge graph completion is framed as a textual entailment task. By aligning the input and output format with a pre-training task, we enable zero-shot transfer, i.e., no training data is required for updating our model. This approach can solve samples that are in the distribution of pre-training corpus. To improve the transfer ability on out-of-distribution samples, we further add light-weighted adapting layers to map the input to pre-training distribution and calibrate the output for knowledge graph completion task. We show the structure of 
% \method\ in Figure \ref{fig:model} and introduce details in the following sections.

% To further improve the transfer ability, we design two kinds of adapting layers, namely \prompt\ and \calibration. The \prompt\ helps to recall related knowledge from the pre-trained language model, and the \calibration\ prepares it for knowledge graph completion. By only tuning these light-weighted layers and keeping all language model parameters fixed, the PLM can efficiently transfer to knowledge graph completion. 
% \subsection{Intuition} \label{sec:intuition}
% The key intuition of \method\ is that the pre-trained language model has already learnt related factual knowledge and we need to recall and prepare such knowledge for knowledge graph completion. For example, to predict whether a given triplet (evening clothes, type of, attire) is correct or not, the necessary knowledge is that attire means ``clothes, especially of a particular or formal type'' and ``evening clothes'' belongs to such type. This is closely related to a natural language understanding task, which motivates us to align the input and output of knowledge graph completion tasks with a language model pre-training task. As a result, we enable zero-shot transfer of BERT for knowledge graph completion, which is shown in the left side of Figure \ref{fig:model}.

% \subsection{Zero-shot Transfer}\label{sec:zero-shot}
% The basis of zero-shot transfer is that knowledge graph completion fits well in textual entailment and the PLM has already learnt related knowledge. For example, to predict whether a given triplet (evening clothes, type of, attire) is correct or not, the necessary knowledge is that attire means ``clothes, especially of a particular or formal type'' and ``evening clothes'' belongs to such type. This is closely related to textual entailment if we take the head entity and relation as premise and the tail entity as hypothesis: 
% \begin{itemize}
%     \vspace{-0.1in}
%     \item[] premise: evening clothes type of
%     \vspace{-0.1in}
%     \item[] hypothesis: attire
%     \vspace{-0.1in}
% \end{itemize}

% In this work, we choose BERT~\cite{BERT} as the PLM. One pre-training task of BERT is next sentence prediction, which aims to predict if a pair of sentences are consecutive, i.e., whether it is natural or not that the first sentence is followed by the second sentence. The textual entailment can be naturally transferred to the same task, if we take the premise as the first sentence and the hypothesis as the second sentence. Specifically, for the previous triplet \texthrt{h} = ``evening clothes'', \texthrt{r} = ``type of'' and \texthrt{t} = ``attire'', we concatenate the text description of head and relation to serve as the first sentence, and tail description as the second sentence, and add special tokens to align the input with pre-training:
% \begin{center}
%     \textspt{[CLS]} evening clothes type of \textspt{[SEP]} attire \textspt{[SEP]}
% \end{center}

% where \textspt{[SEP]} and \textspt{[CLS]} are special tokens designed for pre-training. There is a binary classifier on top of the final representation of \textspt{[CLS]} for next sentence prediction in BERT pre-training, and we directly take the output score of this classifier as the possibility of the input triplet being correct. By aligning the input and output format with pre-training, we enable zero-shot transfer of BERT for knowledge graph completion tasks.

% \subsection{Parameter-efficient Adapting}\label{sec:adapting}
% The zero-shot \method\ can only solve samples that are in the distribution of pre-training corpus. For out-of-distribution samples, we further add two kinds of adapting layers, namely \prompt\ and \calibration . The \prompt\ maps the input representation into the pre-training distribution so that related knowledge can be recalled while the \calibration s prepare such knowledge for knowledge graph completion tasks. 

% \paragraph{Knowledge Prompt Encoder.}
% To recall related knowledge information that might contain in the pre-trained language model, we insert new prompt tokens into the input sequences. As shown in Figure \ref{fig:model}, we choose three positions to add: before the head entity, after the relation and before the tail entity. The embedding of prompt tokens are randomly initialized and are learned during knowledge graph completion training. Furthermore, we add a linear layer with a skip-connection on top of the token embedding layer to project the original token embeddings to another subspace. This projection may help the language model to better align with the pre-training distribution and leverage its knowledge in the following attention layers:
% \begin{align}
%     e_i &= e(x_i) \\
%     e'_i &= W*e_i + b + e_i
% \end{align}
% where $E$ is the embedding matrix, $x_i$ is the token id of $i$th token, and $W$ and $b$ are tunable weight and bias of the linear projection. This differs from prompt-tuning which only inserts prompt tokens into the input.

% \paragraph{Knowledge Calibration Encoder.}
% The original output layer during pre-training is for semantic representation and has a different distribution as the output of knowledge graph completion. Therefore, we need to calibrate it before use for the knowledge graph completion task. To be more specific, we add \calibration s to transform hidden states of the middle and the last Transformer layers. The \calibration s are tuned on knowledge graph completion tasks so that they narrow the distribution mismatch between the output of PLMs and knowledge graph completion. They can be the same as FFN layers which also transform hidden states for the next layer, but we choose linear mapping with a  skip-connection instead since we find that linear mapping is sufficient to achieve good performance and it is more efficient. 

% \subsection{Training}
% \jianhao{more clear description, e.g., introducing the loss}
% To train the adapting layers of \method, we keep all language model parameters fixed and only tune the \prompt\ and \calibration s. we use a negative sampling loss~\cite{negativesample} for each part of a triplet. To be more specific, for a positive triplet (h, r, t), we first corrupt its head entity with $n_\text{ns}$ other random sampled entities to form negative triplets ($\tilde{h}$, r, t). If a sampled triplet is in the knowledge graph, it should be considered as positive so we re-sample it. The loss function for the head entity is:
% \begin{equation}
% \begin{aligned}
%     L_\texthrt{h} = - &\log\Pr(1|h, r, t) \\
%     - &\sum_{i}^{n_\text{ns}} \mathbb{E}_{\tilde{h}_i\sim E \backslash \{h\}}\log \Pr(0 | \tilde{h}_i, r, t)
% \end{aligned}
% \end{equation}
% where $\Pr(\cdot|h, r, t)$ is the output probability of the NSP classifier.

% The same is done to the tail entity and relation, so in total we sample $3*n_\text{ns}$ negative triplets for each positive triplet. The final loss function is the sum of three negative sampling losses:

% \begin{equation}\label{eq:ns}
%     L = L_\texthrt{h} + L_\texthrt{r} + L_\texthrt{t}
% \end{equation}


% \iffalse
% \method\ encodes text description of entities and relations with a modified pre-trained language model for knowledge graph completion, and in this work we use BERT in particular. 
% \subsection{BERT}\label{sec:bert}
% \jianhao{merge necessary information into our method}
% BERT~\cite{BERT} is a widely-used pre-trained language model build with Transformer layers~\cite{Vaswani_attention}. Each Transformer layer consists of two sub-layers: a multi-head attention layer (MHA) and a fully-connected feed-forward layer (FFN). In MHA, the hidden state of each token is updated by a self-attention function, which retrieves related information from other tokens and adds it up. This attention function can be formulated as:
% \begin{align}
%     A &= \frac{QK^{\top}}{\sqrt{d_k}} \\
%     \text{Attention}(Q,K&,V) = \text{softmax}(A)V
% \end{align}

% In FFN, each hidden state is transformed to get prepared for the next layer:
% \begin{equation}
%     \text{FFN}(x) = \sigma(xW_1+b_1)W_2+b_2
% \end{equation}
% where $\sigma$ is the activation function.

% BERT is pre-trained on large corpus with two self-supervised tasks, namely masked language modeling (MLM) and next sentence prediction (NSP). MLM is to recover some masked tokens given other tokens in the sentence. NSP aims to predict if a pair of sentences are consecutive, i.e., whether it is natural or not that the first sentence is followed by the second sentence. For NSP, a special tokens \textspt{[SEP]} is added at the middle of two sentences and another one at the end to mark the boundary. Another special token \textspt{[CLS]} is added at the beginning, serving as a information collector to gather useful representation. There is a binary classifier on top of the final representation of \textspt{[CLS]} for NSP which we refer as the NSP classifier.

% % \subsection{\method}\label{sec:method}
% The key intuition of \method\ is that the pre-trained language model has already learnt related factual knowledge and we need to transfer this knowledge efficiently. We first formulate knowledge graph completion as a standard natural language understanding task, and thus enable zero-shot transfer of BERT for knowledge graph completion. 
% \fi
% To achieve better transfer, we further add two kinds of parameter-efficient adapting layers to the PLM, namely \prompt\ and \calibration.
% Intuitively, the \prompt\ helps to recall related knowledge from the pre-trained language model, and the \calibration\ prepares it for knowledge graph completion. We show the structure of adapting layers in the right side of Figure \ref{fig:model}.


% To retrieve related knowledge efficiently, we design a \prompt, where we insert prompt tokens into the text description and add a linear projection layer after the token embedding to transfer the semantic embedding space. After that, we use two linear layers to calibrate the knowledge before the attention computing, which we call a \calibration. We show the model architecture in Figure \ref{fig:model} and introduce details in the following sections.
